Inferring diffusivity from killed diffusion

We consider diffusion of independent molecules in an insulated Euclidean domain with unknown diffusivity parameter. At a random time and position, the molecules may bind and stop diffusing in dependence of a given `binding potential'. The binding process can be modeled by an additive random functional corresponding to the canonical construction of a `killed' diffusion Markov process. We study the problem of conducting inference on the infinite-dimensional diffusion parameter from a histogram plot of the `killing' positions of the process. We show first that these positions follow a Poisson point process whose intensity measure is determined by the solution of a certain Schr\"odinger equation. The inference problem can then be re-cast as a non-linear inverse problem for this PDE, which we show to be consistently solvable in a Bayesian way under natural conditions on the initial state of the diffusion, provided the binding potential is not too `aggressive'. In the course of our proofs we obtain novel posterior contraction rate results for high-dimensional Poisson count data that are of independent interest. A numerical illustration of the algorithm by standard MCMC methods is also provided.

==> macros.tex <==
% RN commands

\renewcommand{\P}{\mathbb{P}}
\renewcommand{\H}{\mathbb{H}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\W}{\mathbb{W}}
\newcommand{\G}{\mathscr{G}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mW}{\mathcal{W}}
\newcommand{\mB}{\mathcal{B}}
\renewcommand{\L}{\mathscr{L}}
\newcommand{\supp}{\text{supp}}
\newcommand{\var}{\text{Var}}
\newcommand{\eps}{\varepsilon}
\newcommand{\norm}[1]{\left| \left|#1\right| \right|}
\newcommand{\snorm}[1]{| | #1 | |}
\newenvironment{enumerate*}%


\newcommand{\ind}[1]{1\!\!1_{#1}} %\ind{}: independence symbol
\def\iid{\overset{\textnormal{iid}}{\sim}} % i.i.d. symbol

\newcommand{\qmarks}[1]{``#1''} % quotation marks

% Mathematical spaces and objects
\def\B{\mathbb{B}}\def\C{\mathbb{C}}\def\E{\mathbb{E}}\def\H{\mathbb{H}}\def\N{\mathbb{N}}\def\P{\mathbb{P}}\def\R{\mathbb{R}}\def\V{\mathbb{V}}\def\X{\mathbb{X}}\def\W{\mathbb{W}}\def\Z{\mathbb{Z}}\def\1{\mathbbm{1}}

\def\Acal{\mathcal{A}}\def\Bcal{\mathcal{B}}\def\Ccal{\mathcal{C}}\def\Dcal{\mathcal{D}}\def\Ecal{\mathcal{E}}\def\Fcal{\mathcal{F}}\def\Gcal{\mathcal{G}}\def\Hcal{\mathcal{H}}\def\Lcal{\mathcal{L}}\def\Ncal{\mathcal{N}}\def\Ocal{\mathcal{O}}\def\Rcal{\mathcal{R}}\def\Scal{\mathcal{S}}\def\Tcal{\mathcal{T}}\def\Vcal{\mathcal{V}}

\def\Enorm{\textnormal{E}}\def\Covnorm{\textnormal{Cov}}\def\Varnorm{\textnormal{Var}}

\def\Gscr{\mathscr{G}}\def\Xscr{\mathscr{X}}

